Decentralized Statistical Inference with Unrolled Graph Neural Networks

In this paper, we investigate the decentralized statistical inference problem, where a network of agents cooperatively recover a (structured) vector from private noisy samples without centralized coordination. Existing optimization-based algorithms suffer from issues of model mismatch and poor convergence speed, and thus their performance would be degraded, provided that the number of communication rounds is limited. This motivates us to propose a learning-based framework, which unrolls well-noted decentralized optimization algorithms (e.g., Prox-DGD and PG-EXTRA) into graph neural networks (GNNs). By minimizing the recovery error via end-to-end training, this learning-based framework resolves the model mismatch issue. Our convergence analysis (with PG-EXTRA as the base algorithm) reveals that the learned model parameters may accelerate the convergence and reduce the recovery error to a large extent. The simulation results demonstrate that the proposed GNN-based learning methods prominently outperform several state-of-the-art optimization-based algorithms in convergence speed and recovery error.

==> CDC2021 (3)/section/exp.tex <==
\input{section/simulation_snr}
\section{Experiments}\label{sec:experiments}
In this section, we conduct experiments to demonstrate the effectiveness of LProx-DGD and LPG-EXTRA, compared with  Prox-DGD and PG-EXTRA as the baselines, in solving the decentralized sparse vector recovery problem \eqref{prob:lasso}. 

\subsection{Settings}
For the following experiments, the dataset contains 1000 samples for training, 100 samples for validation, and 100 samples for testing. In each sample, the communication graph is generated  randomly by choosing from the set of all graphs with $\lvert \mathcal{V}\rvert = N=5$ nodes and $\lvert \mathcal{E}\rvert = 6$ edges. We let $m\in\{80,300\}$, $m_i = m/N$ and $d_i=100$ and then sample the entries of the sensing matrix $A_i\in \mathbb{R}^{m_i\times 100}\sim\mathcal{N}(\mathbf{0},I)$ and the entries of noise $\epsilon_i\sim \mathcal{N}(\mathbf{0},\sigma^2 I)$ for each agent $i\in\mathcal{V}$, where $\sigma$ is related to the signal-to-noise ratio (SNR) defined as
\begin{align*}
    \text{SNR} = 10 \log_{10}\left(\frac{\mathbb{E}\|x^*\|_2^2 }{\sigma^2} \right).
\end{align*} The sparse ground-truth vector $x^*$ is decided to be nonzero entries following a  Bernoulli-Gaussian distribution with $p_s = m/(2N)$, while the values of nonzero entries also follow the standard normal distribution. 

The recovery error is evaluated by the Normalized Average Mean Square Error (NAMSE) in dB:

\begin{equation}
   \text{NAMSE}(\mathbf{x}^k,\mathbf{x}^*) =10\log_{10}\frac{\mathbb{E}\|\mathbf{x}^k-\mathbf{x}^*\|_F^2} {N \cdot\mathbb{E}\|\mathbf{x}^*\|_F^2},
\end{equation}
for the $k$-th unrolled layer or iteration. We employ NAMSE as the evaluation metric of the following experiments.


We train the learning-based methods for 500 epochs with batch training samples, using the Adam\cite{kingma2015adam} method. For the optimization-based methods, we let the metropolis matrix be $W$ for Prox-DGD and further set $\tilde{W} = \frac{I+W}{2}$ for PG-EXTRA in the following experiments. 

\subsection{Convergence Performance}



We use 50-unrolling-step LProx-DGD and LPG-EXTRA, and compare them to the original forms of Prox-DGD and PG-EXTRA. Since the learning-based methods are data-driven, we fine-tune the fixed parameters in Prox-DGD and PG-EXTRA using validation samples for all the following experiments. However, the process of fine-tuning by grid search methods is tedious and expensive, since the performance is sensitive to the step-size $\alpha$ and the regularization parameter $\lambda$ (cf. Appendix \ref{sec:difficult_tune}). 


Figure \ref{fig:convergence}  plots the convergence performance of  Prox-DGD, PG-EXTRA, LProx-DGD and LPG-EXTRA in terms of NAMSE, for different SNRs and the number of measurements. Observe that LProx-DGD and LPG-EXTRA perform similarly, while both of them significantly outperform  Prox-DGD and PG-EXTRA in  convergence speed. When the number of total measurements is sufficient and the noise level is low (cf. Figure \ref{fig:m300_con_snr50}), the learning-based methods  achieve similar level recovery errors with much fewer iterations. When the number of total measurements is insufficient or the noise level is medium (cf. Figures \ref{fig:m80_con_snr30}-\ref{fig:m80_con_snr50}), the learning-based methods can achieve both faster convergence and smaller recovery errors. This is owing to the learning of a tailored and iteration-wise $\lambda$.


%Such performance implies that learning-based methods can effectively reduce the number of iterations to achieve an even better recovery accuracy. Compared to LProx-DGD, LPG-EXTRA 
%is more stable and less sensitive to different SNRs. In Figure \ref{fig:m80_con_snr30} and \ref{fig:m80_snr_pg}, the number of total samples $m=80$ is less than  the dimension of the recovery problem $d=100$, which makes impossible to converge to the optimal estimator in a linear rate. However, thanks to the learning-based methods, LPG-EXTRA shows its superior convergence speed in the cases of limited measurement samples.



\subsection{Robustness to Noise Levels}
To show that the promising performance of LProx-DGD and LPG-EXTRA is robust to the various levels of noises, we compare their final NAMSEs at different SNRs for recovery problems with different sizes. For each of the following experiments, we unroll each of the learning-based algorithms with $10$ layers and $50$ layers respectively, and compare them to their original forms for $10$, $50$ and $200$ iterations. The results are shown in Figure \ref{fig:SNR}.



Figures \ref{fig:m80_snr_dgd} and \ref{fig:m300_snr_dgd} plot the final recovery errors of LProx-DGD and Prox-DGD with different unrolled iterations at various SNRs, for $m=80$ and $m=300$ respectively.  Similarly, Figure \ref{fig:m80_snr_pg} and \ref{fig:m300_snr_pg} plot those of LPG-EXTRA and PG-EXTRA. Observe that the final recovery errors of LProx-DGD and LPG-EXTRA with $10$ (resp. $50$) unrolled layers are comparable to those of Prox-DGD and PG-EXTRA with $50$ (resp. $200$) iterations, at different levels of noises in both cases of $m=80$ and $m=300$.

Such appealing performance substantiates that the learned parameters can remarkably reduce the number communication rounds by up to $80\%$ compared to the original forms, while guaranteeing the same level of recovery errors given different noisy measurements.

\subsection{Impact of Training Samples}
Deep learning-based methods often require a large number of training samples, which is infeasible to obtain in practice. In this subsection, we show the impact of sample size  on the performance, under the setting of $m=300$ in the last two subsections. As is revealed in Table \ref{tab:sample}, the trained model performs well with only tens of samples. This is achieved by introducing a strong inductive bias into the model.


\begin{table}[htbp]
	
	%\centering  
	\selectfont  
	\centering
	
	\caption{Performance (NAMSE in dB) for  LProx-DGD and LPG-EXTRA with different numbers of training samples.} 
	
	\resizebox{0.46\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|c|}  
			\hline  
 Training Samples & 1 & 5 & 10 & 20 & 50 & 100 & 1000 \\ \hline
 LProx-DGD-10 & -9.99 & -14.17 & -14.74 & -14.59 & -14.77 & -16.98 & -17.65 \\ \hline
 LPG-EXTRA-10 & -11.74 & -14.04 & -14.87 &    -15.19 & 15.41 & -16.73 & -17.17\\ \hline
 LProx-DGD-50 & -30.98 & -34.51 & -34.75 & -35.39 & -35.87 & -36.22 & -38.17 \\ \hline
 LPG-EXTRA-50 & -32.57 & -34.77 & -35.07 &   -35.71 &  -35.96 & -36.07& -36.43\\ \hline

			
	\end{tabular}}
	\label{tab:sample}
\end{table}

==> CDC2021 (3)/section/lasso.tex <==
\section{Application to Decentralized LASSO}\label{sec:algdevelop}
Based on the observations and the general principle developed in the last section, we propose a couple of learning-based methods applying to the decentralized LASSO problem as a running example.
\subsection{LASSO and Algorithms}\label{sec:lasso_alg}
In decentralized LASSO, we have
\begin{align*}
    y_i = A_i x^* + \epsilon_i, \quad \|x^*\|_0 \leq p,
\end{align*}
where $A_i \in \mathbb{R}^{m_i \times d}$ and $m_i$ is the number of measurements for agent $i$. We let $m = \sum_{i=1}^N m_i$ denote the number of total measurements  and further suppose $m_i\ll d$ so that $A_i$ is highly ill-conditioned and each agent $i$ fails to recover $x^*$ independently for $i\in\mathcal{V}$.  This problem has a wide range of applications, e.g., the activity detection in distributed MIMO \cite{guo2020sparse} and distributed feature selection \cite{talwar2015nearly}. To cooperatively estimate the sparse vector $x^*$ in a distributed manner, a common formulation is 

%A typical approach is to employ decentralized optimization algorithms to solve the following  problem:
%A typical approach is to employ $l_1$-norm to encourage the sparse structure of the estimated signal and then to formulate the signal recovery problem as a follow:
%\begin{equation}\label{prob:lasso_centralized}
%\hat{x} :=\underset{x \in \mathbb{R}^d}{\arg\min}  \sum_{i=1}^N \left(\frac{1}{2}\|A_ix - y_i\|_2^2 + \lambda \|x\|_1\right),
%\end{equation}
%where $\lambda$ is the nonnegative penalty parameter that controls the tradeoff between the least-square term and the sparsity regularization term. The problem \eqref{prob:lasso_centralized} is known as the least absolute shrinkage and selection operator (LASSO) in statistics literature \cite{tibshirani1996regression}, which can be solved in a centralized manner. 

\begin{equation}\label{prob:lasso}
\begin{aligned}
&\underset{x_i \in \mathbb{R}^d\ \forall i \in\mathcal{V}}{\text{minimize}} & & \sum_{i=1}^N \left(\frac{1}{2}\|A_ix_i - y_i\|_2^2 + \lambda \|x_i\|_1\right)\\
&\text{subject to}& & x_1 = \cdots = x_N,
\end{aligned}
\end{equation}
where $x_i$ is the local estimate or inference for agent $i\in\mathcal{V}$.  The equality constraint of \eqref{prob:lasso} enforces the optimal estimates of the agents to achieve a consensus denoted by $\hat{x}\in\mathbb{R}^d$.
 
To match the formulation of \eqref{prob:compact}, we let $\mathbf{s}(\mathbf{x}) = \sum_{i=1}^N \frac{1}{2}{\|A_ix_i-y_i\|_2^2}$ and $\mathbf{r}(\mathbf{x}) = \sum_{i=1}^N \|x_i\|_1$. Then, we are able to apply the following decentralized optimization algorithms mentioned in Section \ref{subsec:decentralized} to the decentralized LASSO, i.e.,  problem \eqref{prob:lasso}.

\textbf{Prox-DGD for LASSO:}  Each agent $i\in\mathcal{V}$ starts from an arbitrary initial point $x_i^0\in\mathbb{R}^d$, and then for each $ k\ge 0$, updates according to
\begin{align} 
    x_i^{k + \frac{1}{2}} = &\sum_{j = 1}^N w_{ij} x^{k}_j  - \alpha^k A_i^T (A_i x_i^{k} - y_i), \label{eq:dgd_lasso0}\\
     x^{k+1}_i = & \mathcal{S}_{\alpha^k\lambda}(x_i^{k + \frac{1}{2}}), \label{eq:dgd_lasso1}
\end{align}
where $\mathcal{S}_a(x)$ is  the soft-thresholding operator with the threshold $aI$. Specifically, 
$\mathcal{S}_{\alpha^k\lambda}(x) = \text{ReLU}(x - \alpha^k \lambda I) - \text{ReLU}( - x - \alpha^k \lambda I)$, which coincides with the ReLU component of the GCN introduced in Section \ref{subsec:gnn}.

\textbf{PG-EXTRA for LASSO:} Each agent $i\in\mathcal{V}$ chooses an arbitrary initial point $x_i^0\in\mathbb{R}^d$  and then for each $k\ge 0$, updates according to \begin{align}x_i^{\frac{1}{2}} =& \sum_{j=1}^N w_{ij}x_j^0\! -\! \alpha A_i^T(A_ix_i^0-y_i), &&\text{if } k=0,\label{eq:pg_lasso_init0}\\
x_i^{1} =& \mathcal{S}_{\alpha\lambda}(x_i^{ \frac{1}{2}}),& & \text{if } k=0;\label{eq:pg_lasso_init1}\\
    x_i^{k + \frac{1}{2}} = &\sum_{j = 1}^N w_{ij} x^{k}_j + x^{k - \frac{1}{2}}_i \!-\! \sum_{j=1}^N \Tilde{w}_{ij} x^{k-1}_j  \notag\\
    & - \alpha  A_i^T A_i (x_i^{k} - x_i^{k-1}) ,  &&\text{if } k>0, \label{eq:pg_lasso0}\\
    x^{k+1}_i = & \mathcal{S}_{\alpha\lambda}(x_i^{k + \frac{1}{2}}),&&\text{if } k>0. \label{eq:pg_lasso1}
\end{align}

%x_hat noteq x^*
Note that Prox-DGD and PG-EXTRA are able to converge to the optimal consensus  $\hat{x}$ of problem \eqref{prob:lasso}, under proper assumptions on the step-sizes and the  mixing matrices. However, the LASSO estimator $\hat{x}$ is different from the ground-truth vector $x^*$ that we expect to recover. In fact, both of the above algorithms perform poorly on LASSO in terms of convergence speed and recovery accuracy in practice, which motivates us to employ learning-based methods to overcome such drawbacks.

%Insipred , we will discuss how to embed the decentralized algorithms into the architecture of GNNs and how to learn the model paramters automatically.

%Notice that there are two kinds of parameters appearing the the above updates: the step size $\alpha$ and the penalty parameter $\lambda$. In our model, both of these parameters will be learned by GNNs automatically. In the sequel, we will describe the reasons why these parameters are crucial to improve the convergency speed and recovery error.


\subsection{Recovery Error Analysis}\label{sec:convergence_analysis}
A natural question is what should be learned to improve the performance. To answer this question, we present the recovery error analysis for PG-EXTRA as an example to justify the learning of the step-sizes and the regularization parameters. We impose the standard assumptions in the analysis of decentralized algorithms  \cite{shi2015pgextra} and compressive sensing \cite{chandrasekaran2012convex,oymak2013squared}.

\begin{assumption}\label{assump:mixingmatrix}
The mixing matrices $W = [w_{ij}]\in\mathbb{R}^{N\times N}$ and $\tilde{W} = [\tilde{w}_{ij}]\in\mathbb{R}^{N\times N}$ 
are symmetric and satisfy $[w_{ij}],[\tilde{w}_{ij}]>0\  \forall j\in\mathcal{N}_i\cup \{i\}$, and $[w_{ij}]=[\tilde{w}_{ij}] = 0$ otherwise. Also, $\text{null}\{W-\tilde{W}\} = \text{span}\{\mathbf{1}\}$ and $\text{null}\{I-\tilde{W}\} \supseteq \text{span}\{\mathbf{1}\}$. Moreover, $\tilde{W}\succeq \mathbf{O}$ and $\frac{I+W}{2}\succeq \tilde{W}\succeq W$.
\end{assumption}

\begin{assumption}\label{assump:measurematrix} For $i\in\mathcal{V}$, the entries of
$A_i \sim \mathcal{N}(\mathbf{0}, I)$ and the entries of $\epsilon_i \sim \mathcal{N}(\mathbf{0},\sigma_i^2 I)$.
\end{assumption}


Note that Assumption \ref{assump:mixingmatrix} ensures that each agent only interacts with its neighbors and implies that $\lambda_{\max}(\tilde{W}) = 1$. For the following analysis, we first claim some notations as follows: We denote $\mathbf{x}^* = (x^*,\ldots,x^*)^T\in\mathbb{R}^{N\times d} $ and $\hat{\mathbf{x}} = (\hat{x},\ldots,\hat{x})^T\in\mathbb{R}^{N\times d}$. Suppose that there exists $\hat{\mathbf{q}}\in\mathbb{R}^{N\times d}$ satisfying

 $$(\tilde{W}-W)^{\frac{1}{2}}\hat{\mathbf{q}}+\alpha(\nabla\mathbf{s}(\hat{\mathbf{x}}) + \lambda\tilde{\nabla} \mathbf{r}(\hat{\mathbf{x}})) = \mathbf{O}.$$
Then, let $\mathbf{q}^k = \sum_{t=0}^k (\tilde{W}-W)^{\frac{1}{2}}\mathbf{x}^t$, $\hat{\mathbf{z}} = ((\hat{\mathbf{q}})^T, (\hat{\mathbf{x}})^T)^T$, and $\mathbf{z}^k = ((\mathbf{q}^k)^T, (\mathbf{x}^k)^T)^T$.



The following theorem shows that the recovery error at the $k$-th iteration has an upper bound. 

%The recovery error consists of two parts: the error between achieved solution and the optimal solution to \eqref{prob:lasso}, and the error between the optimal solution to \eqref{prob:lasso} and the ground-truth signal $x^*$. 


\begin{theorem} \label{thm:rec}
Suppose that Assumptions \ref{assump:mixingmatrix} and \ref{assump:measurematrix} hold. Let  $L_s = \max_i \lambda_{\max}(A_i^TA_i)$ and $\sigma = \max_{i} \sigma_i$.
If $m > O(p\log(d/p))$ and $\alpha < \frac{2\lambda_{\min}(\tilde{W})}{L_s}$, then
\begin{align*} \label{eq:conv}
    \|\mathbf{x}^{k+1} - \mathbf{x}^*\|_{\tilde{W}}^2  \leq & 2 \|\mathbf{z}^{0} - \hat{\mathbf{z}}\|^2_{G} - 2\sum_{t = 0}^{k}\xi \|\mathbf{z}^{t+1} - \mathbf{z}^{t}\|^2_{G} \nonumber\\
    &+ \mathcal{O}_{\mathbb{P} }\left(\frac{\sigma^2 Np\max\{ \log d,  \lambda^2\}  }{m}     \right),
\end{align*}
where $\xi = 1 - \alpha L_s/(2\lambda_{\min}(\tilde{W}))$ and $G = \left(\begin{array}{cc}
I & \mathbf{O} \\
\mathbf{O} & \tilde{W}
\end{array}\right)$.
\end{theorem}
\begin{proof}
See Appendix \ref{proof:rec}.
\end{proof}

Theorem \ref{thm:rec} provides an error upper bound of the recovery error generated by PG-EXTRA at the $k$-th iteration. To improve the performance, it is better to let the optimal $\alpha$ and $\lambda$ vary across iterations and problem settings. Such flexibility leads to a linear increase of hyperparameters, which are very difficult to fine-tune\footnote{We verify the difficulty of tuning parameters in Appendix \ref{sec:difficult_tune}.}. Therefore, adaptive sequences of step-sizes and regularization coefficients can achieve a better error bound compared to the fixed one. 



\subsection{Learning-based Algorithms}\label{sec:learning_based_framework}
Following the general principle in Section \ref{subsec:unrolling}, the remaining part is to determine the learnable parameters and the loss function. Motivated by the recovery error analysis in the last subsection, we set $\alpha^k$ and $\lambda^k$ as the learnable parameters, where $k$ is the iteration index. 

Next, we develop the loss function, which aims to ensure that each step has a sufficient descent. To do so, we set the loss function as a weighted sum of the distances between the $k$-th unrolled iteration's output and the ground-truth $\mathbf{x}^*$, for all $k$, i.e.,
 \begin{equation}\label{eq:loss_func}
   \ell(\Theta) = \sum_{k = 1}^K  \gamma^{K-k} \|\mathbf{x}^k(\Theta) - \mathbf{x}^* \|_F^2,
\end{equation}
where $\Theta = \{\lambda_i, \alpha_i\}_{1 \leq i \leq K}$ groups the learnable parameters, $K$ is the total number of unrolled iterations and $\gamma\le 1$ is a discounting factor.

%Then, the graph neural networks induced by unrolled Prox-DGD and PG-EXTRA are shown in Algorithm \ref{alg}.

The learning-based PG-EXTRA is shown in Algorithm \ref{alg}. 

\begin{algorithm}[H]
\caption{Learned PG-EXTRA (LPG-EXTRA)}
 \label{alg}
\begin{algorithmic}[1]
 \STATE Each node $i\in\mathcal{V}$ arbitrarily chooses the initial $x_i^{0}\in\mathbb{R}^d$.
\FOR{$k=0,1,\ldots$}
\STATE $\lambda \gets \lambda_{nn}(k)$.
\STATE $\alpha \gets \alpha_{nn}(k)$.
\STATE Each node $i \in \mathcal{V}$ sends $x_i^k$ to every neighbor $j \in \mathcal{N}_i$.
\STATE Upon receiving $x_j^k$ $\forall j\in \mathcal{N}_i$, each node $i\in \mathcal{V}$ updates  $x_i^{k+\frac{1}{2}}$ and $x_i^{k+1}$  according to \eqref{eq:pg_lasso_init0}-\eqref{eq:pg_lasso1}.
\ENDFOR
\end{algorithmic}
\end{algorithm}
\begin{rem}
The functions $\lambda_{nn}(k)$ and $\alpha_{nn}(k)$ represent the learned parameters outputted by the $k$-th layer of the graph neural network.
\end{rem}
\begin{rem}
The learned Prox-DGD (LProx-DGD) differs from Algorithm \ref{alg} only at the $6$-th line, where the updates of LProx-DGD are given by  \eqref{eq:dgd_lasso0} and  \eqref{eq:dgd_lasso1}.
\end{rem}
\input{section/simulation_con}
During the training, the ground-truth vector $x^*$ is required to be available for all the agents to learn the parameters, but it is definitely not needed for testing. Guided by minimizing the loss function, agents are enforced to emulate the ground-truth vector within $K$ iterations. In the sequel, we illustrate via a number of experiments that the learned algorithms perform excellently for a family of input measurements and ground-truth vectors.









==> CDC2021 (3)/section/obv_unrolling.tex <==

\section{Unrolling Decentralized Optimization Algorithms into Graph Neural Networks }\label{sec:relation and unrolling}
%1. Introduce the distributed opt problems, detailed formulation\\
%2. point out its convex problem and mention the existing algorithms used later.\\
%3. Claim the limitation of existing alg\\
%4. Our methods....


In this section, we introduce classic decentralized optimization algorithms to solve \eqref{prob:compact}  in Section \ref{subsec:decentralized}. We then illustrate the message passing schemes of GNNs and their relationships to decentralized optimization algorithms in Section \ref{subsec:gnn}, and describe the general guidelines of unrolling approaches in Section \ref{subsec:unrolling}.

%. The underlying relationship between decentralized optimization algorithms and GNNs is revealed  together with the general guidelines of unrolling approaches.


\subsection{Decentralized Optimization Algorithms}\label{subsec:decentralized}


%We suppose that a set $\mathcal{V} = \{1,2,\ldots,N\}$ of agents  and their interactions  form a networked multi-agent system, which can be modeled as an undirected and connected \textit{communication graph} $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where $\mathcal{E} \subseteq \{\{i,j\}:i,j\in\mathcal{V},i\ne j\}$ represents the set of channels. Each agent $i\in\mathcal{V}$ can communicate directly  with its (one-hop) neighbors, i.e., $\mathcal{N}_i=\{j\in\mathcal{V}:\{i,j\}\in\mathcal{E}\}$. Assume that each agent $i$ is endowed with a local objective function $f_i: \mathbb{R}^d\to\mathbb{R}+\cup\{+\infty\}$ such that 
%\begin{equation*}
%    f_i(x) = s_i(x) + r_i(x),
%\end{equation*}
%where each $s_i:\mathbb{R}^d\to \mathbb{R}$ is a convex and differentiable function whose gradient is Lipschitz continuous, and each $r_i: \mathbb{R}^d\to \mathbb{R}\cup \{+\infty\}$ is a convex and but possibly nondifferentiable function.


%Then, all the $N$ agents cooperatively minimize the sum of their local  objectives in the following composite form:
%\begin{equation}\label{eq_composite}
%   \underset{x\in\mathbb{R}^d}{ \operatorname{minimize}} \sum_{i=1}^N (s_i(x)+r_i(x)).
%\end{equation}
A  number of decentralized optimization algorithms have been proposed to solve composite optimization problems in the form of \eqref{prob:compact}. To handle the nonsmooth term in problem  \eqref{prob:compact}, one typical approach is to incorporate a proximal operation into certain decentralized first-order algorithms. Below, we present a few classic and state-of-the-art examples of the existing algorithms, which will be embedded into our proposed GNN-based learning framework later and further serve as baselines in our experiments.



\textbf{Prox-DGD:} Prox-DGD \cite{zeng2018proxdgd} incorporates the proximal operator with the decentralized gradient descent (DGD) algorithm \cite{nedic2009dgd}, which is able to handle nonconvex, nonsmooth optimization problems. It operates as follows: Starting from an arbitrary initial point $\mathbf{x}^{0}\in\mathbb{R}^{N\times d}$, and the update equations are given by
\begin{align*}
\mathbf{x}^{k+\frac{1}{2}} = & W\mathbf{x}^k - \alpha^k \nabla \mathbf{s}(\mathbf{x}^k), && \forall k\ge 0,\\
\mathbf{x}^{k+1} =& \prox_{\alpha^k\lambda \mathbf{r}}(\mathbf{x}^{k+\frac{1}{2}}), &&\forall k\ge 0,
\end{align*}
where $\alpha^k> 0$ is the step-size at the iteration $k$  and $W=[w_{ij}]\in\mathbb{R}^{N\times N}$ is the mixing matrix satisfying  \cite[Assumption 2]{zeng2018proxdgd}, which enables the decentralized implementation, i.e., $w_{ij} = 0$ if $i\ne j$ and $\{i,j\}\notin \mathcal{E}$, and $w_{ij}>0$ otherwise.

\textbf{PG-EXTRA:} PG-EXTRA~\cite{shi2015pgextra} is a decentralized proximal gradient method, which is an extension of the decentralized exact first-order algorithm (EXTRA) \cite{shi2015extra}. 
It starts from an arbitrary initial point $\mathbf{x}^0\in\mathbb{R}^{N\times d}$ and then the entire network of agents update as follows:
\begin{align*}
\mathbf{x}^{\frac{1}{2}} =& W\mathbf{x}^{0} - \alpha \nabla \mathbf{s}(\mathbf{x}^0), & & \\
\mathbf{x}^{1} =& \prox_{\alpha\lambda\mathbf{r}}(\mathbf{x}^{\frac{1}{2}});&&\\
\mathbf{x}^{k+1+\frac{1}{2}}=& W \mathbf{x}^{k+1}+\mathbf{x}^{k+\frac{1}{2}}-\tilde{W} \mathbf{x}^{k}&& \nonumber\\
&-\alpha\left[\nabla \mathbf{s}(\mathbf{x}^{k+1})-\nabla \mathbf{s}(\mathbf{x}^{k})\right], &&\forall k\ge 0,\\
\mathbf{x}^{k+2} =& \prox_{\alpha\lambda\mathbf{r}}(\mathbf{x}^{k+1+\frac{1}{2}}), &&\forall k\ge 0,
\end{align*}
where $\alpha>0$ is the step-size. In addition, $W = [w_{ij}]\in\mathbb{R}^{N\times N}$ and $\tilde{W} = [\tilde{w}_{ij}]\in\mathbb{R}^{N\times N}$ are mixing matrices satisfying \cite[Assumption 1]{shi2015pgextra}, which will be discussed in Section \ref{sec:convergence_analysis} detailedly. 

%\textbf{NIDS} NIDS~\cite{li2019nids }is closedly related to PG-EXTRA  but using uncoordinated step sizes. Given arbitrary $x_i^{(0)}\in\mathbb{R}^d$ and its own step size $\alpha_i>0$, let $x_{i}^{(\frac{1}{2})}= x_{j}^{(0)}-\alpha_i \nabla s_{i}(x_{i}^{(0)})$ and $x_i^{(1)} = \prox_{\alpha_i\lambda r_i}(x_i^{(\frac{1}{2})})$, for 
%each agent $i\in\mathcal{V}$. Then, each agent $i$ performs 
%\begin{align}
%x_{i}^{(k+1+\frac{1}{2})}=& x_i^{(k+\frac{1}{2})} - x_i^{(k+1)} + \sum_{j=1}^N \tilde{w}_{ij}\left(2x_j^{(k+1)} - x_j^{k} - \right.\nonumber\\
%&\left.-\alpha_j\left[\nabla s_{j}(x_{j}^{(k+1)})-\nabla s_{j}(x_{j}^{(k)})\right]\right),\\
%x_i^{(k+2)} =& \prox_{\alpha_i\lambda r_i}(x_i^{(k+1+\frac{1}{2})}),
%\end{align}
%where $k>0$ and $W = [w_{ij}] \in\mathbb{R}^{N\times N}$ satisfies 

Note that the updates of the above two algorithms can be summarized by the following three procedures at each iteration: (\romannum{1}) Each agent $i$ mixes its decision variable $x_i^k$ with its neighbors' information by particular mixing matrices, when $(x_1^k,\ldots,x_N^k)^T = \mathbf{x}^k$.  (\romannum{2}) Each agent $i$ takes advantage of the  first-order information of $s_i$ (i.e., $\nabla s_i$) to update. (\romannum{3}) Each agent $i$ performs the proximal 
mapping of $r_i$.

We take Prox-DGD as an example to illustrate the above iterative procedure in Figure \ref{fig:dop}, which will be compared with the graph convolutional networks in the next subsection.


%For instance, the Lasso, $l_1$-regularized linear regression, is widely used in distributed sparse channel estimation \cite{channelestimation_Zaib16} and distributed compressed sensing problem \cite{}. 


\subsection{Graph Neural Networks}\label{subsec:gnn}
In classic machine learning tasks (e.g., image processing), data can be typically embedded into the Euclidean space and thus convolutional neural networks show their competent performance. Recently, there is an increasing number of non-Euclidean applications such as point clouds, molecule structures, and complex networks. These data can be naturally modeled as graphs, and efforts have been put forward to develop neural networks applicable to graphs \cite{wu2019comprehensive}.

Like other deep architectures, graph neural networks (GNNs) have a layer-wise architecture. In each layer of a GNN, every node updates its representation by aggregating features from its neighbors. Specifically, suppose that the graph of a GNN is the same as the aforementioned  \textit{communication graph} $\mathcal{G}$ in Section \ref{sec:sysmodelandmotivations}. Then, the update rule of the $k$-th layer at node $i\in\mathcal{V}$ in a GNN \cite{xu2018powerful} is
\begin{align} \label{eq:gnn}
    x_i^{k+1} = \psi^{k}\left(x_i^{k}, \phi^{k}\left( \left\{ x_j^{k} : j \in \mathcal{N}_i \right\}\right) \right),
\end{align}
where $x_i^k$ denotes the feature vector of node $i$, $\phi^k$ is the aggregation function of node $i$ that collects information from the neighboring nodes, and $\psi^k$ is the function that combines the aggregated information with node $i$'s own information. GNNs in the form of \eqref{eq:gnn} can be implemented efficiently with Pytorch Geometric \cite{fey2019fast}.

One of the popular GNNs is the graph convolutional network (GCN) \cite{kipf2016semi}. The update of a GCN can be written as the following compact form:
\begin{align}
    \mathbf{x}^{k+1} = \text{ReLU}\left(L \mathbf{x}^{k}\Theta  + \mathbf{b}\right),
\end{align}
where ReLU is a nonlinear activation function,  $L\in\mathbb{R}^{N\times N}$ is the Laplacian matrix of the graph $\mathcal{G}$ (which also can induce the decentralized implementation like mixing matrices) and $\Theta\in\mathbb{R}^{d\times d}, \mathbf{b}\in\mathbb{R}^{N\times d}$ are the trainable weights.
%where $L = D^{-\frac{1}{2}} A D^{-\frac{1}{2}}$ is the graph Laplacian matrix, $A$ is the adjencency matrix with self-loop, $D$ is the degree matrix of $A$, $\{\Theta, b_i\}$ is a trainable weights.

The similarities between the GCN and Prox-DGD are shown in Fig \ref{fig:dopgnn}. Note that the operation of both Prox-DGD and PG-EXTRA can be written in the general form of a GNN update as in \eqref{eq:gnn}: Let $\phi^k(\cdot)$ be a \textit{weight sum} aggregation function and $\psi^k(\cdot)$ represents other operations like a gradient descent followed by a proximal mapping. 




\subsection{Unrolling Decentralized Algorithms into GNNs}\label{subsec:unrolling}
As classic decentralized algorithms such as Prox-DGD and PG-EXTRA can be cast into the form of GNNs (\ref{eq:gnn}), we may implement these algorithms by the deep graph learning toolbox \cite{fey2019fast}. In the classic optimization algorithms, the hyperparameters need to be manually tuned to achieve desirable performance. With the assistance of data-driven methods, the parameters in the problem formulation and the algorithm (e.g., $\alpha^k$, $\lambda$ and $W$ in the updates of Prox-DGD) can be automatically learned by adopting the recovery error as the loss function. Specifically, denoting $\Theta$ as the set of learnable parameters in the GNN and $\mathbf{x}^{k+1}(\Theta, \{f_i, y_i\}_{i\in\mathcal{V}})$ as the output of the unrolled GNN in the $k$-th layer,  a general form of the loss function can be written as 
\begin{align} \label{loss:gen}
    \ell(\Theta) = d\left(\mathbf{x}^{k+1}(\Theta, \{f_i, y_i\}_{i\in\mathcal{V}}),x^*\right),
\end{align}
where $d(\cdot,\cdot)$ is some distance metric. 

The learning-based algorithm consists of two stages. In the training stage, we collect a number of training samples, i.e., the pair of $(\{f_i, y_i\}_{i\in\mathcal{V}}, x^*)$, and optimize the GNN's learnable parameters by (sub)gradient descent with the objective in \eqref{loss:gen}. In the test stage, the trained neural network is applied and we use the \textit{forward} function in \cite{fey2019fast} to run the algorithms. As the GNNs are implemented by distributed message-passing \cite{fey2019fast}, the update of one node only requires its neighbors' information. As a result, it naturally runs in a decentralized manner.

==> CDC2021 (3)/section/simulation_con.tex <==
\begin{figure*}[htbp]
    \centering
    \subfigure[SNR $=30$ and $m=80$.]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m80DGD30.eps}
        \label{fig:m80_con_snr30}
    }
    \subfigure[SNR $= 30$ and $m=300$.]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m300snr30.eps}
        \label{fig:m300_con_snr30}
    }
    \subfigure[SNR $=50$ and $m=80$.]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m80snr50.eps}
        \label{fig:m80_con_snr50}
    }
    \subfigure[SNR $=50$ and $m=300$.]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m300snr50.eps}
        \label{fig:m300_con_snr50}
    }
        \caption{Convergence performance of LProx-DGD and LPG-EXTRA compared with the original forms of Prox-DGD and PG-EXTRA with fine-tuned parameters, for SNR $= 30,50$ and $m=80,300$, respectively. }
    \label{fig:convergence}
\end{figure*}


==> CDC2021 (3)/section/simulation_snr.tex <==
\begin{figure*}[htbp]
    \centering
    \subfigure[Prox-DGD and LProx-DGD ($m = 80$).]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m80_dgd.eps}
        \label{fig:m80_snr_dgd}
    }
    \subfigure[Prox-DGD and LProx-DGD ($m = 300$).]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m300_dgd.eps}
        \label{fig:m300_snr_dgd}
    }
    \subfigure[PG-EXTRA  and LPG-EXTRA ($m = 80$).]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m80_PG.eps}
        \label{fig:m80_snr_pg}
    }
    \subfigure[PG-EXTRA and LPG-EXTRA ($m = 300$).]
    {
        \includegraphics[width=0.47\columnwidth]{fig/m300snr.eps}
        \label{fig:m300_snr_pg}
    }
        \caption{Performance of  LProx-DGD and LPG-EXTRA, compared with Prox-DGD, PG-EXTRA with fine-tuned parameters, under different SNRs. The left two figures show the final recovery errors (evaluated by NAMSE) of LProx-DGD and Prox-DGD, while the right two figures present those of  LPG-EXTRA and PG-EXTRA, with different unrolled layers or iterations.}
    \label{fig:SNR}
\end{figure*}

==> CDC2021 (3)/section/sysmodel.tex <==
\section{Problem Formulation}\label{sec:sysmodelandmotivations}
Suppose a set $\mathcal{V} = \{1,2,\ldots,N\}$  of agents  and their interactions form a networked multi-agent system, which is modeled as an undirected and connected \textit{communication graph} $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where $\mathcal{E} \subseteq \{\{i,j\}:i,j\in\mathcal{V},i\ne j\}$ represents the set of communication links. Agent $i\in\mathcal{V}$ can only communicate   with its (one-hop) neighbors, denoted by $\mathcal{N}_i=\{j\in\mathcal{V}:\{i,j\}\in\mathcal{E}\}$. 

The goal of all the agents is to  cooperatively recover a (structured) vector $x^* \in \mathbb{R}^d$ from their noisy measurements. Each agent $i\in\mathcal{V}$ is associated with its own estimate vector $x_i\in\mathbb{R}^d$ of $x^*$ and its local measurement $y_i \in\mathbb{R}^{m_i}$, in the form of
\begin{equation*}
    y_i = f_i(x^*) + \epsilon_i,
\end{equation*}
where $f_i:\mathbb{R}^d\to\mathbb{R}^{m_i}$ is the measurement or sampling function of agent $i$, and $\epsilon_i\in \mathbb{R}^{m_i}$ is the measurement noise by agent $i$. This setting is prevalent in communication and machine learning. For example, in a distributed communication system, $x^*$ denotes the transmit symbol, $f_i$, $y_i$, $\epsilon_i$ denote the channel propagation, the received symbol, and the addictive noise of the channel at the $i$-th receiver, respectively \cite{zaib2016distributed,guo2020sparse}. In distributed private learning, $x^*$ is the optimal model weight, $f_i$ is the data-generating process, $y_i$ is the label and $\epsilon_i$ is the sampling noise in data \cite{he2018cola,talwar2015nearly}. 

Due to the limited number of measurements and the presence of noise, it is impossible for each agent to recover $x^*$ on its own. In the decentralized setting, each agent only maintains its own measurements and the recovering objective function privately. Unlike the centralized statistical inference approaches, there is no data fusion center that collects data or measurements from agents.  To recover $x^*$ in a coordinated way, each agent $i\in\mathcal{V}$ is allowed to communicate with its neighbors, such as its latest local estimate.

A typical approach is to formulate the recovery problem as the following composite programming problem:
\begin{equation}\label{prob:composite}
\begin{aligned}
&\underset{x_i \in \mathbb{R}^d\ \forall i\in\mathcal{V}}{\text{minimize}} & & \sum_{i=1}^N \left(s_i\left(x_i \right) + \lambda r_i(x_i)\right)\\
&\text{subject to}& & x_1 = \cdots = x_N,
\end{aligned} 
\end{equation}
where each $s_i(x_i) = h_i(f_i(x_i); y_i)$ is a function measuring the distance between $f_i(x_i)$ and $y_i$, each $r_i(x_i)$ is a regularizer revealing the underlying structure of the optimal solution $x^*$ (i.e., the vector to be recovered) and $\lambda$ is a nonnegative scalar. Suppose that each $s_i:\mathbb{R}^{d}\to \mathbb{R}$ is a convex differentiable function whose gradient is Lipschitz continuous, and each $r_i: \mathbb{R}^d\to \mathbb{R}\cup \{+\infty\}$ is a convex and proximable but possibly nondifferentiable function. Note that  $r_i$ is allowed to include an indicator function $I_{X_i}$, with respect to any closed convex set $X_i$, so that problem \eqref{prob:composite} can be constrained by $x_i\in X_i$.


Indeed, many real-world engineering problems can be cast into problem \eqref{prob:composite}. In the setting of decentralized compressive sensing, $s_i$ is squared $\ell_2$ distance, and $r_i$ is the $\ell_1$-norm (if $x^*$ is sparse) \cite{tibshirani1996regression} or nuclear norm (if $x^*$ is low-rank) \cite{candes2010power}. In the setting of distributed learning, $s_i$ is often the cross-entropy or support vector machine (SVM) loss, and $r_i$ is the $\ell_1$-norm or Euclidean norm.

%For instance, suppose $y_i = A_ix^* +z_i$, where $A_i\in\mathbb{R}^{m_i\times d}\ \forall i\in\mathcal{V}$ is a linear transformation matrix and $z_i$ is an additive Guassian white noise. We have $\sum_{i=1}^N m_i\ll d$ such that it is  a highly ill-posed system. To recover the sparse signal $x^*$, let $s_i(x_i) = \|A_ix_i - y_i\|_2^2$ and $ r_i(x_i) = \|x_i\|_1$. Then, problem \eqref{prob:composite} is a decentralized $l_1$-regularized least squares problem or LASSO (least-absolute shrinkage and selection operator) for) in a decentralized setting.
\begin{figure*} 
\subfigure[An illustration of Prox-DGD in the compact form.]{
\begin{minipage}[t]{0.48\linewidth}
\includegraphics[width = 0.95\textwidth,trim=100 100 100 100,clip]{fig/dopfig2.pdf}
\label{fig:dop}
\end{minipage}
}
\subfigure[An illustration of GCN in the compact form.]{
\begin{minipage}[t]{0.48\linewidth}
\centering
\includegraphics[width = 0.95\textwidth,trim=100 100 100 100,clip]{fig/gnnfig2.pdf}
\label{fig:gcn}
\end{minipage}
}
\caption{The similarities between Prox-DGD \cite{zeng2018proxdgd} and the GCN  \cite{kipf2016semi}. Interestingly, ReLU is the proximal mapping of $I_{\{\mathbf{x}\in\mathbb{R}^{N\times d}|\mathbf{x} \geq \mathbf{O}\}}(\mathbf{x})$.
}
\label{fig:dopgnn}
\end{figure*}

In the following analysis, we denote $\mathbf{x} = (x_1,x_2,\ldots,x_N)^T\in\mathbb{R}^{N\times d}$ and
$S = \{\mathbf{x}\in\mathbb{R}^{N\times d}: x_1 = x_2 = \cdots = x_N\}$. Then,
we  rewrite problem \eqref{prob:composite} as the following compact form:
\begin{equation}\label{prob:compact}
\begin{aligned}
&\underset{\mathbf{x} \in \mathbb{R}^{N\times d}}{\text{minimize}} & & \mathbf{s}(\mathbf{x}) + \lambda\mathbf{r}(\mathbf{x})\\
&\text{subject to}& & \mathbf{x}\in S,
\end{aligned} 
\end{equation}
where $\mathbf{s}(\mathbf{x}) = \sum_{i=1}^N s_i(x_i)$ and  $\mathbf{r}(\mathbf{x}) = \sum_{i=1}^N r_i(x_i)$.

%\subsection{Motivations}
%Formulating the problem into \eqref{prob:compact} and solving it with existing algorithms, e.g., PG-EXTRA \cite{shi2015pgextra}, face some limitations. First, minimizing  \eqref{prob:compact} does not directly minimize the recovery error, since the formulation is based on convex relation.

%Second, the optimal regularization parameter $\lambda$ should vary from problem to problem in order to achieve the best recovery results, which increase the difficulty to find a suitable formulation of problem \eqref{prob:compact}. Third, in order to achieve the best convergence speed, the parameters in the algorithms, e.g., the step size at each iteration, should be hard to determine, which causes expensive costs to optimally tune parameters in an iteration-wised manner.

%One solution is to treat the optimization process as a black-box and directly use a neural network to output the final solution \cite{li2019graph,gama2020graph,shen2020graph}.

%use a neural network under the multi-agent setting to approximate the input pair of existing centralized algorithm. The 

%to use a neural network under the multi-agent setting \cite{gama2020graph,shen2020graph} as they are trained in an end-to-end manner by directly optimizing the recovery error. Nevertheless, the convergence cannot be guaranteed and 


%One can solve the above mentioned issues by designing a neural network and employing 

%Motivated by these issues, we propose to design a neural network to solve composite optimization problem \eqref{prob:composite}, or equivalently problem \eqref{prob:compact}.


%The problem formulation (\ref{prob:compact}) is often based on convex relaxation. As a result, the optimal parameter $\lambda$ varies from problem to problem. Second, to achieve the best convergence speed, the parameters in the algorithm, e.g., step size in each step, should be optimally tuned in an iteration-wised manner. 



